The Key to Deobfuscation is Pattern of Life, not Overcoming Encryption

Preserving privacy is an undeniable benefit to users online. However, this benefit (unfortunately) also extends to those who conduct cyber attacks and other types of malfeasance. In this work, we consider the scenario in which Privacy Preserving Technologies (PPTs) have been used to obfuscate users who are communicating online with ill intentions. We present a novel methodology that is effective at deobfuscating such sources by synthesizing measurements from key locations along protocol transaction paths. Our approach links online personas with their origin IP addresses based on a Pattern of Life (PoL) analysis, and is successful even when different PPTs are used. We show that, when monitoring in the correct places on the Internet, DNS over HTTPS (DoH) and DNS over TLS (DoT) can be deobfuscated with up to 100% accuracy, when they are the only privacy-preserving technologies used. Our evaluation used multiple simulated monitoring points and communications are sampled from an actual multiyear-long social network message board to replay actual user behavior. Our evaluation compared plain old DNS, DoH, DoT, and VPN in order to quantify their relative privacy-preserving abilities and provide recommendations for where ideal monitoring vantage points would be in the Internet to achieve the best performance. To illustrate the utility of our methodology, we created a proof-of-concept cybersecurity analyst dashboard (with backend processing infrastructure) that uses a search engine interface to allow analysts to deobfuscate sources based on observed screen names and by providing packet captures from subsets of vantage points.

==> Makefile <==
PRJ = 2023-x-scoped-tda

LATEX = pdflatex -shell-escape

all: pdf

$(PRJ):
	$(LATEX) $(PRJ) && bibtex $(PRJ) ; $(LATEX) $(PRJ).tex && $(LATEX) $(PRJ).tex

pdf: $(PRJ) 
#	dvipdf $(PRJ).dvi

ps: $(PRJ)
	latex $(PRJ) && bibtex $(PRJ) && latex $(PRJ) && dvips -P cmz -t letter -G0 -o $(PRJ).ps $(PRJ).dvi

view : ${PRJ}.pdf
	open ${PRJ}.pdf &
	
spell: 
	for i in `grep -v "^%" $(PRJ).tex |perl -e 'while(<>){chomp;$$s=$$_;if($$s=~m/input\{([^}]+)}/){print $$1, "\n"}}'`; do aspell -c -x -t $${i}; done

count:
	@grep -v "^%" $(PRJ).tex |perl -e 'while(<>){chomp;$$s=$$_;if($$s=~m/input{([^}]+)}/){print $$1, "\n"}}' | xargs cat $(TEX_FILES) | grep -v "^%" | wc

outline:
	$(LATEX) outline.tex

clean:
	rm -f *.aux *.dvi *.log *.pdf *.ps *.bbl *.blg


